MaskMedPaint: Masked Medical Image Inpainting with Diffusion Models for Mitigation of Spurious Correlations

Spurious features associated with class labels can lead image classifiers to rely on shortcuts that don't generalize well to new domains. This is especially problematic in medical settings, where biased models fail when applied to different hospitals or systems. In such cases, data-driven methods to reduce spurious correlations are preferred, as clinicians can directly validate the modified images. While Denoising Diffusion Probabilistic Models (Diffusion Models) show promise for natural images, they are impractical for medical use due to the difficulty of describing spurious medical features. To address this, we propose Masked Medical Image Inpainting (MaskMedPaint), which uses text-to-image diffusion models to augment training images by inpainting areas outside key classification regions to match the target domain. We demonstrate that MaskMedPaint enhances generalization to target domains across both natural (Waterbirds, iWildCam) and medical (ISIC 2018, Chest X-ray) datasets, given limited unlabeled target images.

==> tables/cxr_dataset_split.tex <==
\begin{table}[H]
\begin{center}
\begin{tabular}{lllll}
\toprule
\multirow{2}{*}{} & Source & \multicolumn{3}{c}{Target} \\
 & MIMIC & CheXpert & PadChest & NIH \\
 \midrule
Train & 10000 & - & - & - \\
Val & 1000 & - & - & - \\
Extra & - & 1000 & 1000 & 1000 \\
Test & 2000 & 2000 & 2000 & 2000 \\
\bottomrule
\end{tabular}    
\end{center}
\caption{Dataset splits for CXR images}
\label{table:cxr_dataset_split}
\end{table}

==> tables/iwildcam_grayscale-to-color_animal.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lllllll}
\toprule
\textbf{Model} & \textbf{cattle} & \textbf{elephants} & \textbf{impalas} & \textbf{zebras} & \textbf{giraffes} & \textbf{dik-diks} \\
\midrule
Train Prevalence & 48\% & 8\% & 21\% & 6\% & 4\% & 7\% \\
OOD Test Prevalence & 15\% & 17\% & 21\% & 6\% & 33\% & 6\% \\
\midrule
Base & 0.892 & 0.029 & 0.071 & 0.250 & 0.223 & 0.250 \\
CutMix & 0.983 & 0.000 & 0.024 & 0.125 & 0.045 & 0.083 \\
MixUp & 0.983 & 0.029 & 0.000 & 0.042 & 0.280 & 0.000 \\
MaskMedPaint & 0.583 & 0.162 & 0.000 & 0.396 & 0.826 & 0.771 \\
\bottomrule
\end{tabular}
\caption{Dataset prevalences and test OOD accuracy of methods across the predicted animal classes for the grayscale to color shift.}
\label{table:grayscale-to-color_animal}
\end{table*}

==> tables/iwildcam_night-to-day_animal.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lllllll}
\toprule
\textbf{Model} & \textbf{cattle} & \textbf{elephants} & \textbf{impalas} & \textbf{zebras} & \textbf{giraffes} & \textbf{dik-diks} \\
\midrule
Train Prevalence & 0\% & 9\% & 19\% & 17\% & 8\% & 35\% \\
OOD Test Prevalence & 47\% & 7\% & 23\% & 10\% & 1\% & 4\% \\
\midrule
Base & 0.186 & 0.000 & 0.033 & 0.050 & 0.000 & 0.750 \\
CutMix & 0.245 & 0.000 & 0.000 & 0.075 & 0.000 & 0.875 \\
MixUp & 0.053 & 0.000 & 0.098 & 0.175 & 0.000 & 0.750 \\
MaskMedPaint & 0.005 & 0.286 & 0.103 & 0.700 & 0.000 & 0.906 \\
\bottomrule
\end{tabular}
\caption{Dataset prevalences and test OOD accuracy of methods across the predicted animal classes for the night to day shift.}
\label{table:night-to-day_animal}
\end{table*}
